Feed-forward Uncertainty Propagation in Belief and Neural Networks

We propose a feed-forward inference method applicable to belief and neural networks. In a belief network, the method estimates an approximate factorized posterior of all hidden units given the input. In neural networks the method propagates uncertainty of the input through all the layers. In neural networks with injected noise, the method analytically takes into account uncertainties resulting from this noise. Such feed-forward analytic propagation is differentiable in parameters and can be trained end-to-end. Compared to standard NN, which can be viewed as propagating only the means, we propagate the mean and variance. The method can be useful in all scenarios that require knowledge of the neuron statistics, e.g. when dealing with uncertain inputs, considering sigmoid activations as probabilities of Bernoulli units, training the models regularized by injected noise (dropout) or estimating activation statistics over the dataset (as needed for normalization methods). In the experiments we show the possible utility of the method in all these tasks as well as its current limitations.

==> style/tex_defs1.tex <==
%\usepackage{mathrsfs}
\DeclareMathAlphabet{\mathcalligra}{T1}{calligra}{m}{n}
\DeclareMathAlphabet{\mathantt}{OT1}{antt}{li}{it}
\DeclareMathAlphabet{\mathpzc}{OT1}{pzc}{m}{it}

\DeclareMathOperator{\Path}{path}
\DeclareMathOperator{\aff}{aff}
\DeclareMathOperator{\opt}{opt}
\newcommand{\Argmax}{\mathop{\rm Argmax}}
\newcommand{\argmax}{\mathop{\rm argmax}}
\newcommand{\Argmin}{\mathop{\rm Argmin}}
\newcommand{\argmin}{\mathop{\rm argmin}}
\DeclareMathOperator{\Arg}{Arg}
\DeclareMathOperator{\rank}{rank}
\DeclareMathOperator{\Row}{Row}
\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Col}{Col}
\DeclareMathOperator{\ort}{^{\bot}}
\DeclareMathOperator{\dom}{dom}
\DeclareMathOperator{\ri}{relint}
\DeclareMathOperator{\conv}{conv}
\DeclareMathOperator{\coni}{coni}
\DeclareMathOperator{\Null}{null}
\DeclareMathOperator{\select}{select}

\let\oldemptyset\emptyset
\let\emptyset\varnothing

\newcommand{\<}{\langle}
\renewcommand{\>}{\rangle}
\newcommand{\Mid}{\:\big|\,}
\renewcommand{\mid}{\:|\,}
\newcommand{\bb}{\boldsymbol}

\newcommand{\Real}{\mathbb{R}}
%\newcommand{\WI}{\ensuremath{{\rm WI}(\Lambda,f)}\xspace}
%\newcommand{\SI}{\ensuremath{{\rm SI}(\Lambda,f)}\xspace}
%\newcommand{\WIg}{\ensuremath{{\rm WI}(\Lambda,g)}\xspace}
%\newcommand{\SIg}{\ensuremath{{\rm SI}(\Lambda,g)}\xspace}
%\newcommand{\WIx}[1]{\ensuremath{{\mathbb{W}}(\Lambda,#1)}\xspace}
%\newcommand{\SIx}[1]{\ensuremath{{\mathbb{S}}(\Lambda,#1)}\xspace}
%\newcommand{\WI}{\ensuremath{{\mathbb{W}}(\Lambda,f)}\xspace}
%\newcommand{\SI}{\ensuremath{{\mathbb{S}}(\Lambda,f)}\xspace}
%\newcommand{\WIg}{\ensuremath{{\mathbb{W}}(\Lambda,g)}\xspace}
%\newcommand{\SIg}{\ensuremath{{\mathbb{S}}(\Lambda,g)}\xspace}

\newcommand{\WIx}[1]{\ensuremath{\mathbb{W}_{#1}}\xspace}
\newcommand{\SIx}[1]{\ensuremath{\mathbb{S}_{#1}}\xspace}
\newcommand{\WI}{\WIx{f}}
\newcommand{\SI}{\SIx{f}}
\newcommand{\WIg}{\WIx{g}}
\newcommand{\SIg}{\SIx{f}}


\newcommand{\Natural}{\mathbb{N}}
\newcommand{\bbN}{\mathbb{N}}
\newcommand{\bbZ}{\mathbb{Z}}
\newcommand{\bbQ}{\mathbb{Q}}
\newcommand{\Rationals}{\mathbb{Q}}

\def\bbbone{{\mathchoice {\rm 1\mskip-4mu l} {\rm 1\mskip-4mu l}{\rm 1\mskip-4.5mu l} {\rm 1\mskip-5mu l}}}
\newcommand{\Ind}{\bbbone}
\newcommand{\tab}{{\hphantom{bla}}}
\newcommand{\A}{\mathcal{A}}
\newcommand{\Bool}{\mathbb{B}}
\newcommand{\Boolean}{\mathbb{B}}
\newcommand{\bigU}{\mathbb{U}}
\newcommand{\B}{\mathcal{B}}
\newcommand{\D}{\mathcal{D}}
\def\O{\mathcal{O}}
\newcommand{\F}{\mathcal{F}}
\def\G{\mathcal{G}}
\def\H{\mathcal{H}}
\newcommand{\mF}{\mathcal{F}}
\newcommand{\mP}{\mathcal{P}}
\newcommand{\mC}{\mathcal{C}}
\def\C{\mathcal{C}}
\newcommand{\Literals}{\mathbb{\nLabels}}
\newcommand{\V}{\mathcal{V}}
\newcommand{\I}{\mathcal{I}}
\def\U{\mathcal{U}}
\newcommand{\W}{\mathcal{W}}
\renewcommand{\P}{\mathcal{P}}
\newcommand{\E}{\mathcal{E}}
\DeclareMathOperator{\sym}{sym}
\newcommand{\EE}{\tilde{\E}}
\newcommand{\N}{\mathcal{N}}
\newcommand{\X}{\mathcal{X}}
\newcommand{\Y}{\mathcal{Y}}
\newcommand{\calH}{\mathcal{H}}
\newcommand{\calS}{\mathcal{S}}
\newcommand{\calI}{\mathcal{I}}
\renewcommand{\L}{\mathcal{L}}
\newcommand{\M}{\mathcal{M}}
%\newcommand{\LL}{\bb{\mathcal{L}}}
\newcommand{\LL}{\mathcal{X}}
\newcommand{\Labels}{\X}
\newcommand{\nLabels}{L+1}
%\newcommand{\vect}{\overrightarrow}
%\newcommand{\lvect}{\overleftarrow}
\def\T{^{\mathsf T}}
\newcommand{\st}{\mbox{s.t.\ }}

\newcommand{\bulletpar}{\noindent $\bullet\tab$}
\newcounter{myRomanCounter}
\newcommand*{\RomanItem}[1]{\setcounter{myRomanCounter}{#1}\par\noindent\Roman{myRomanCounter}.\ }
\newcommand*{\RomanNumber}[1]{\setcounter{myRomanCounter}{#1}\Roman{myRomanCounter}}

\providecommand{\Zeta}{\mathcal{Z}}

%\def\etalb{{\itshape \bfseries et al.}}
%\def\etalb{{\itshape et al.}}
\def\etalb{ et al.}
\newcommand{\f}{{E_f}}
\newcommand{\g}{{E_g}}
\newcommand{\h}{{E_h}}
\newcommand{\x}{{x}}
\newcommand{\y}{{y}}
\newcommand{\z}{{z}} 
\newcommand{\w}{{w}}

%\newcommand{\sE}{{\scriptsize \textrm{E}}}
%\newcommand{\sG}{{\scriptsize \textrm{G}}}
%\newcommand{\sH}{{\scriptsize \textrm{H}}}

%\newcommand{\c}{{\scriptstyle \textrm{C}}}
%\newcommand{\sD}{{\scriptstyle \textrm{D}}}
%\newcommand{\sH}{{\scriptstyle \textrm{H}}}


%\newcommand{\c}{\textsc{c}}
%\newcommand{\c}{\textsc{c}}
\def\c{\textsc{c}}
\def\d{\textsc{d}}
\def\h{\textsc{h}}
\def\a{\textsc{a}}
\def\b{\textsc{b}}
\def\j{\textsc{j}}
%\newcommand{\sD}{\textsc{d}}
%\newcommand{\sH}{\textsc{h}}

%\newcommand{\c}{\textsc{j}}
%\newcommand{\sD}{\textsc{k}}
%\newcommand{\sH}{\textsc{h}}

\newcommand{\Esubset}{\stackrel{.}{\subsetneq}}
\newcommand{\Esubseteq}{\stackrel{.}{\subset}}
\newcommand{\Esupset}{\stackrel{.}{\supsetneq}}

\newcommand{\Gsubset}{\stackrel{..}{\subsetneq}}
\newcommand{\Gsupset}{\stackrel{..}{\supsetneq}}


%\newcommand{\sE}{e}
%\newcommand{\sG}{c}
%\newcommand{\sH}{d}

\newcommand{\energy}[1]{{E_{#1}}}
\newcommand{\bc}{{\bf c}}
\newcommand{\bzero}{0}
\newcommand{\bone}{1}
\newcommand{\K}{\mathcal{K}}

\newcommand{\nx}{\overline{x}}
\newcommand{\define}{:=}
\newcommand{\PD}{\mathbb{S}_{++}}
\newcommand{\PSD}{\mathbb{S}_{+}}

\newcommand*{\LB}{\ensuremath{\mathit LB}\xspace}
\newcommand*{\LBtwo}{\ensuremath{\mathit LB2}\xspace}
\newcommand*{\LBtwodual}{\ensuremath{\mathit LB2\mbox{-}dual}\xspace}
\newcommand*{\LP}{\ensuremath{\mathit LP\mbox{-}1}\xspace}
\newcommand*{\LPtwo}{\ensuremath{\mathit LP\mbox{-}2}\xspace}


\newtheorem{Note}{note}

\newtheorem{method}{Method}

\newcommand{\smallL}{{\scriptscriptstyle{\left(\right.}}}
\newcommand{\smallR}{{\scriptscriptstyle{\left.\right)}}}

\renewcommand{\iff}{{\textrm{iff} }}

\newcommand{\VH}{V{\'a}clav Hlav{\'a}{\v c}}
\newcommand{\AS}{Alexander Shekhovtsov}
\newcommand{\TW}{Tom{\'a}{\v s} Werner\xspace}
\newcommand{\IRTC}{International Research and Training Center\\ for Informational Technologies and Systems, Kiev}
\newcommand{\CMP}{Czech Technical University in Prague,\\
    Faculty of Electrical Engineering, Department of Cybernetics\\
    Center for Machine Perception}
\newcommand{\gray}{\color[rgb]{0.5,0.5,0.5}}
\newcommand{\red}{\color[rgb]{1,0,0}}
\newcommand{\green}{\color[rgb]{0,1,0}}
\newcommand{\blue}{\color[rgb]{0,0,1}}

\newlength{\figwidth}
\newlength{\figwidtha}
\newlength{\figwidthb}

%\newcommand*{\mypar}[1]{\paragraph{#1}}
\newcommand*{\mypar}[1]{\par{\normalsize\bf #1}\ }
\renewcommand*{\paragraph}[1]{\par\noindent{\normalsize\bf #1}\,\xspace}

\renewcommand*{\marginpar}[1]{\marginnote{#1}}


\def\mathrlap{\mathpalette\mathrlapinternal} 
\def\mathllap{\mathpalette\mathllapinternal}
\def\mathllapinternal#1#2{\llap{$\mathsurround=0pt#1{#2}$}}
\def\mathrlapinternal#1#2{\rlap{$\mathsurround=0pt#1{#2}$}}

\def\ij{i,j}
\def\ji{j,i}
\DeclareRobustCommand{\ind}[1]{\vphantom{f}_{#1}}
\DeclareRobustCommand{\ind}[1]{(#1)}

\def\leftbb{\mathrlap{[}\hskip1.3pt[}
\def\rightbb{]\hskip1.36pt\mathllap{]}}

\def\bbleft{\leftbb}
\def\bbright{\rightbb}
\def\barvee{\veebar}
\def\Vee{\bigvee}
\def\Wedge{\bigwedge}
\def\phi{\delta}
\def\epsilon{\varepsilon}
\def\eps{\varepsilon}
\newcommand{\IF}{\mbox{ \rm if }}
\newcommand{\OR}{\mbox{ \rm or }}
\newcommand{\AND}{\mbox{ \rm and }}
\newcommand{\OTHERWISE}{\mbox{ \rm otherwise}}
\newcommand{\Algorithm}[1]{{Algorithm\,\ref{#1}}}
\newcommand{\Algorithms}[1]{{Algorithms\,\ref{#1}}}
\newcommand{\Section}[1]{\cref{#1}}
%\newcommand{\Section}[1]{\S\ref{#1}}
\makeatletter
\let\parSym\S
\def\S{\mathcal{S}}
\makeatother
\newcommand{\Figure}[1]{{Figure\,\ref{#1}}}
\newcommand{\Theorem}[1]{{Theorem\,\ref{#1}}}
\newcommand{\Lemma}[1]{{Lemma\,\ref{#1}}}
\newcommand{\Chapter}[1]{{Chapter\,\ref{#1}}}
\newcommand{\Chapters}[1]{{Chapters\,\ref{#1}}}
\newcommand{\Statement}[1]{{Statement\,\ref{#1}}}
\newcommand{\Corollary}[1]{{Corollary\,\ref{#1}}}
\newcommand{\Definition}[1]{{Definition\,\ref{#1}}}

\setlength{\arraycolsep}{0.2em}

\newcommand{\halfskip}{\vskip0.5\baselineskip}
\def\defeq{\buildrel \text{d{}ef}\over =}	
\newcommand{\lsub}[1]{\limits_{\begin{subarray}{l}\setlength{\arraycolsep}{0.2em}#1\end{subarray}}}
\newcommand{\csub}[1]{\limits_{\begin{subarray}{c}\setlength{\arraycolsep}{0.2em}#1\end{subarray}}}
\newcommand{\clim}[1]{\limits_{\begin{subarray}{c}\setlength{\arraycolsep}{0.2em}#1\end{subarray}}}

\newcommand{\mincut}{{\scshape mincut}\xspace}
\newcommand{\maxflow}{{\scshape maxflow}\xspace}
%\newcommand{\mincludegraphics}[2][]{\includegraphics[#1]{#2}}
\makeatletter
\newenvironment{rsmallmatrix}{\null\,\vcenter\bgroup
  \Let@\restore@math@cr\default@tag
  \baselineskip6\ex@ \lineskip1.5\ex@ \lineskiplimit\lineskip
  \ialign\bgroup\hfil$\m@th\scriptstyle##$&&\thickspace\hfil
  $\m@th\scriptstyle##$\crcr
}{
  \crcr\egroup\egroup\,
}
\makeatother
%
\def\maxwi{\eqref{best L-improving}\xspace}
\def\maxsi{{(\mbox{\sc max-si})}\xspace}
\def\cf{\emph{cf}\onedot} \def\Cf{\emph{Cf}\onedot}

%\def\revisit{\ensuremath{\red \triangle}\xspace}
\newcommand{\revisit}[1][]{%
\ifthenelse{\equal{#1}{}}{% no argument
\ensuremath{\red \triangle}\xspace}{%
{\ensuremath{\red \rhd}\xspace}%
{\gray #1}%
{\ensuremath{\red \lhd}\xspace}%
}%
}

\def\anchor [#1]#2{%
\phantomsection{}#1\label{#2}%
\def\arga{#2}%
\global\expandafter\def\csname#2\endcsname{%
\hyperref[#2]{#1}\xspace%
}%
}%

\def\codefunction [#1]#2{%
\phantomsection{}\label{#2}{\ttfamily #1\xspace}%
\def\arga{#2}%
\global\expandafter\def\csname#2\endcsname{%
\hyperref[#2]{\ttfamily #1}\xspace%
}%
}

\usepackage{array}
\newcolumntype{L}[1]{>{\raggedright\let\newline\\\arraybackslash\hspace{0pt}}m{#1}}
\newcolumntype{C}[1]{>{\centering\let\newline\\\arraybackslash\hspace{0pt}}m{#1}}
\newcolumntype{R}[1]{>{\raggedleft\let\newline\\\arraybackslash\hspace{0pt}}m{#1}}

\def\checkmark{\tikz\fill[scale=0.4](0,.35) -- (.25,0) -- (1,.7) -- (.25,.15) -- cycle;}

\newcommand{\mm}{\mathit{m}}

\SetKwFor{forever}{while true}{}{end while}
\def\peq{\mathrel{{+}{=}}}
\def\meq{\mathrel{{-}{=}}}

\newcommand{\ubar}[1]{\underaccent{\bar}{#1}}

\newcommand{\norm}[1]{\lVert#1\rVert_1}

\newcommand{\footlabel}[2]{%
    \addtocounter{footnote}{1}%
    \footnotetext[\thefootnote]{%
        \addtocounter{footnote}{-1}%
        \refstepcounter{footnote}\label{#1}%
        #2%
    }%
    $^{\ref{#1}}$%
}

\newcommand{\footref}[1]{%
    $^{\ref{#1}}$%
}

\def\epsilon{\varepsilon}

\newcommand{\leqL}{\mathbin{{\leq}_{\text{\tiny{L}}}}}
\newcommand{\leqAP}{\mathbin{{\leq}_{\text{\tiny AP}}}}


==> tex/draft_notes.tex <==
\clearpage
\section{Draft notes}
\subsection{Efficiency}
Our marginalizing model is relatively inexpensive to implement.
Every layer requires twice larger output storage for mean and variance (and their gradients during training). Bernoulli layers can be implemented without this extra storage since the distribution is fully specified by the mean parameter. Univariate functions such as $\Phi$, $\Li_2$ can be well approximated by piece-wise polynomials. Compared to computationally intensive convolutional filters, they should not significantly hinter the performance.

\subsection{Uncertainties}
In our NN model along with estimating the outputs, the uncertainties are propagated in each layer. We consider both: continuous and discrete state hidden units and all common types of non-linearities. Continuous units are non-linear functions of inputs and the uncertainty is propagated to them using a Gaussian distribution model. Discrete units are considered to be random variables conditioned on the inputs. They have associated posterior probability, which depends on the uncertainty of the inputs but may also them-self introduce uncertainties, such as a logistic model in the first hidden layer may be uncertain in its activations.
\paragraph{Limitations} The framework is applicable for models that are suitable for recognition problems, when there is a single true value or class to estimate. A single-mode factorized distribution around the estimate simply provides the mean to more accurately assess the uncertainty of such estimates. In contrast, models that generate e.g. images as their outputs would really have a multi-modal posterior distribution. Here our simple approximation is not useful as it cannot capture possible modes.
We will distinguish two main types of layers: with continuous and discrete variables.


\subsection{Continuous Layers}
The state variable $X \in \Real ^n$ is described by the mean $\mu^X$ and a diagonal covariance matrix $\Sigma^X = \diag(\sigma^X)$.
Examples:
\begin{itemize}
\item Input image with i.i.d. Gaussian noise
\item Output layer with ReLU activation
\item Output layer with linear activation
\end{itemize}
Activations such as ReLU and linear are interpreted as just non-linear mappings of the input variables.

\subsection{Binary Layers}
The state variable is discrete, \ie, $X \in \{0,1\}^n$, and the output of the layer is the associated activation probability $P(X_i = 1)$.
Such layers can represent occurrences of features at all levels (edges, curves, parts of objects, objects, categories). This is often also the desired from of the output in classification problems.
One specific example is logistic regression, a single-layer network estimating posterior conditional  probability of outputs given the inputs.
\par
A Bernoulli distributed random variable $X_i$ with probability $p = P(X_i = 1)$ has associated mean $\mu^{X_i} = p$ and variance $\sigma^{X_i} = p(1-p)$.
\subsection{Categorical Layers}
The state variables are discrete multi-class, $X \in \{0,\dots, K\}^n$. The difference is that the output of such layer is a multi-valued function consisting of probabilities $p(X_i = k)$ for all $k$. Such outputs can be treated, using appropriate lifting, as $K$-tuples of binary random variables, which however clearly cannot be considered independent. 
% Can represent as multivariate logistic distribution?
%In this case the posterior can be described by the mean vector $\mu^{X_i} \in \Real^K$ and covariance matrix $\Sigma^{X_i} \in \Real^{K \times K}$.
%With such outputs we can associate a vector of means $\mu^{X_i} \in \Real^K$ and covariance 
%\afterpage{\clearpage}
%
%
\section{Components}
\paragraph{Plan}
\begin{itemize}
\item best factorized posterior is given by marginals
\item marginals of continuous variables - mean and variance
\item marginals of binary variables - Bernoulli distribution
\item represent all by mean and variance
\item pre-activation is a weighted combination of discrete or real-valued variables and is real-valued with mean and variance
\item discrete activation by hard-thresholding is a binary RV - CDF
\item sigmoid activation is a binary RV - scaled CDF
\item ReLU activation - mean and variance
\item SeLU activation - mean and variance
\item Pooling layers: (average -- linear mapping, L2 -- take Jacobean,
 max-pooling - )
\end{itemize}
%
%


==> tex/experiments.tex <==
\section{Experiments}\label{sec:experiments}
%
%
%
\begin{figure*}[!t]
\resizebox{\linewidth}{!}{
\includegraphics[width=0.25\linewidth]{fig/exps/MLP/v_acc.pdf}\ %
\includegraphics[width=0.25\linewidth]{fig/exps/MLP/stability_acc.pdf}\ %
\includegraphics[width=0.25\linewidth]{fig/exps/MLP/stability_lodds.pdf}\ %
\includegraphics[width=0.25\linewidth]{fig/exps/MLP/stability1_acc.pdf}\ %
}\vspace{1mm}%
\caption{
Single hidden layer of Bernouli-logistic units, MNIST. All networks have similar test accuracy in the noise-free scenario (numbers shown in brackets). Our models (V, V-Norm) have better stability \wrt both the random noise and adversarial perturbations. The normalization improves training speed while not harming stability in this case. Batch normalization of standard network (S-BN) shows much worse stability. 
When it makes errors under noise it does so with a very high confidence as measured by probability odds of the predicted class to the true class.}
\label{fig:onelayer}
\end{figure*}
%
\begin{figure}[!t]
\centering
\includegraphics[width=.8\linewidth]{fig/exps/speed/t_loss.pdf}%
%\vspace{-2mm}%
\caption{Learning speed in case of a difficult deep sigmoid network. The plot shows the negative likelihood of the training set being minimized (solid lines) and validation set (dashed lines). Note that the scale is logarithmic. Standard network learns slowly, experiencing vanishing gradients problem. Batch normalization clearly helps. Our V-Init and V-Norm variants are at least as good as BN.}
\label{fig:learnspeed}
\end{figure}
%
%
%
We verify the conjecture that accounting for uncertainty leads to more robust models and test the performance of normalization. We consider the standard neural network stdNN (denoted {\bf S} in figures), the proposed varNN (denoted {\bf V} in figures) and the respective variants with normalization: {\bf S-BN} (batch normalization) and {\bf V-Norm} (our normalization~\cref{sec:different-layers}).
%address the following questions: speed of learning and stability to random and adversarial perturbations.
Details of the implementation (in pytorch), parameters, models, \etc, can be found in the supplementary~\cref{sec:extraexp}.
%%==========================================================================================
\paragraph{Single Layer Analysis}
Consider a fully connected model with one hidden layer. This classical model, trained on MNIST dataset already reveals quite surprising results. The hidden layer consists of 100 logistic-Bernoulli units, which are treated as stochastic units in varNN and as usual sigmoid activations in stdNN, in order with approximation~\eqref{AP1}.
%Our varNN model was trained assuming the input has a fixed variance 0.1.
Our varNN model has one extra parameter, the assumed variance of the input, which is set to $0.1$ (\cf signal range [0,\,1]). The standard approach to quantify performance is to measure the classification accuracy on the validation set as shown in~\cref{fig:onelayer} left. All models achieve similar accuracies with normalized variants being slightly better, as could be expected.

%In this figure 
%
%One can argue that the behavior of this model can be in correspondence with the behavior of an isolated layer in a deeper network. 
%Standard NN corresponds to the approximation~\ref{AP1} and varNN propagates variance as propo
%We verify the conjecture that improving approximation \ref{AP1} corresponding to stdNN can be improved by 
%If the first experiment we consider a simple case of a single hidden layer. We train 
%
%We analyze and compare the standard neural network (stdNN) with the newly proposed varNN on the the architecture with a single hidden layer. This can be viewed as testing the behavior of a single layer in a deeper network. 
%
%For this we consider a network with a single, fully connected hidden layer with 100 logistic sigmoid units and train it on MNIST. The two variants differ in the approximation used for computing the conditional probabilities of the output units (\ref{AP1} and \ref{AP2b} respectively, see Table~\ref{table:approx}). 
%Each of them has been trained with and without normalization, by using standard batch normalization for stdNN and the normalization described in Sec.~\ref{sec:different-layers} for varNN. The goal of this experiment is to compare the two approaches w.r.t.~validation accuracy and stability against perturbations. The left display in Fig.~\ref{fig:onelayer} shows that both approaches are on par w.r.t.~validation accuracy, which is expected for this simple classification task. Notice that the normalized variants show a somewhat higher accuracy when compared to their counterparts without normalization.
%
The picture changes dramatically when comparing the stability of the learned networks under different types of perturbations. We considered two types of perturbations: (1) Gaussian noise and (2) adversarial perturbations. For the latter we use the gradient sign attack tailored for each image and targeting the misclassification criterion, as provided by \cite{Rauber2017foolbox}. We then count the number of samples that are misclassified with perturbation norm smaller than a given value.
We also measured confidence odds of the networks, defined as the ratio of the predicted class probability over the true one: $\max_y q(y) / q(y^*)$. %The geometric mean of this ratio is computed over the test set (corresponding to average log odds).
 \cref{fig:onelayer} shows that varNN clearly outperforms stdNN in all three criteria. Notice also that batch normalization leads to a severe degradation in the stability of stdNN. This is an interesting phenomenon for further research.
%This is not case for our normalization for varNN. A deeper analysis of this unexpected effect of batch normalization for stdNN is without any doubt necessary, but beyond the scope of this paper. 
%
%%=============================================================================
%
%
%
%
%\begin{figure*}[!t]
%\resizebox{\linewidth}{!}{
%\begin{tabular}{c}%
%\includegraphics[width=0.5\linewidth]{fig/exps/LeNetB/view/t_loss.pdf}%
%\end{tabular}\ %
%\begin{tabular}{c}%
%\includegraphics[width=0.5\linewidth]{fig/exps/LeNetB/view/v_acc.pdf}%
%\end{tabular}\ %
%\begin{tabular}{c}%
%\includegraphics[width=0.5\linewidth]{fig/exps/LeNetB/view/stability_acc.pdf}%
%\end{tabular}\ %
%\begin{tabular}{c}%
%\includegraphics[width=0.5\linewidth]{fig/exps/LeNetB/view/stability1_acc.pdf}%
%\end{tabular}%
%}\vspace{-2mm}%
%\caption{Comparison of stdNN and varNN for CNN with Bernoully units. From left to right: training and validation losses vs.~training epochs, validation accuracy vs.~training epochs, accuracy vs.~unspecific perturbation noise and accuracy vs.~adversarial perturbations. S and S-BN label the the un-normalized and batch normalized versions of stdNN. V and V-Norm label the respective variants of varNN. Constant input variance 0.1 was used when learning the latter. The numbers in brackets indicate the validation accuracy of the respective nets without perturbations.}
%\label{fig:LeNet}
%\end{figure*}
%
%\begin{figure*}[!t]
%\resizebox{\linewidth}{!}{
%\begin{tabular}{c}%
%\includegraphics[width=0.5\linewidth]{fig/exps/ReLU/B_stability_acc.pdf}%
%\end{tabular}\ %
%\begin{tabular}{c}%
%\includegraphics[width=0.5\linewidth]{fig/exps/ReLU/R_stability_acc.pdf}%
%\end{tabular}\ %
%\begin{tabular}{c}%
%\includegraphics[width=0.5\linewidth]{fig/exps/ReLU/B_stability1_acc.pdf}%
%\end{tabular}\ %
%\begin{tabular}{c}%
%\includegraphics[width=0.5\linewidth]{fig/exps/ReLU/R_stability1_acc.pdf}%
%\end{tabular}%
%}\vspace{-2mm}%
%\caption{Comparison of stdNN and varNN for CNN with Bernoully units. From left to right: training and validation losses vs.~training epochs, validation accuracy vs.~training epochs, accuracy vs.~unspecific perturbation noise and accuracy vs.~adversarial perturbations. S and S-BN label the the un-normalized and batch normalized versions of stdNN. V and V-Norm label the respective variants of varNN. Constant input variance 0.1 was used when learning the latter. The numbers in brackets indicate the validation accuracy of the respective nets without perturbations.}
%\label{fig:LeNet}
%\end{figure*}
%
%
%
\begin{figure*}[!t]
\resizebox{\linewidth}{!}{
\begin{tabular}{c}%
\includegraphics[width=0.5\linewidth]{fig/exps/CIFAR/view/t_loss.pdf}%
\end{tabular}\ %
\begin{tabular}{c}%
\includegraphics[width=0.5\linewidth]{fig/exps/CIFAR/view/v_acc.pdf}%
\end{tabular}\ %
\begin{tabular}{c}%
\includegraphics[width=0.5\linewidth]{fig/exps/CIFAR/view/stability_acc.pdf}%
\end{tabular}\ %
\begin{tabular}{c}%
\includegraphics[width=0.5\linewidth]{fig/exps/CIFAR/view/stability1_acc.pdf}%
\end{tabular}%
}%\vspace{-2mm}%
\caption{Results for CIFAR and conv network with 9 layers and logistic-Bernoulli units. S and V networks get stuck with vanished gradients.
Our normalized version performs better than BN in all objectives, but is not very robust in the absolute scale.
}
\label{fig:CIFAR}
\end{figure*}
%
%
%
\begin{figure}[!t]
\resizebox{\linewidth}{!}{
\begin{tabular}{c}
\footnotesize Accuracy vs Gaussian noise\\
\begin{tabular}{c}%
\includegraphics[width=0.5\linewidth]{fig/exps/ReLU/B_stability_acc.pdf}%
\end{tabular}\ %
\begin{tabular}{c}%
\includegraphics[width=0.5\linewidth]{fig/exps/ReLU/R_stability_acc.pdf}%
\end{tabular}\\[-4pt]%
\footnotesize Accuracy vs adversarial attack\\
\begin{tabular}{c}%
\includegraphics[width=0.5\linewidth]{fig/exps/ReLU/B_stability1_acc.pdf}\\[-4pt]%
\footnotesize Sigmoid
\end{tabular}\ %
\begin{tabular}{c}%
\includegraphics[width=0.5\linewidth]{fig/exps/ReLU/R_stability1_acc.pdf}\\[-4pt]%
\footnotesize ReLU
\end{tabular}\\%
%
\end{tabular}
}%\vspace{-2mm}%
\caption{
Stability of LeNet with logistic-Bernoulli and ReLU activations. Under Gaussian noise our models have better stability than stdNN, for both activations. %Using logistic-Bernoulli activations we get better stability to adversarial attacks. 
Under adversarial attacks we only observe better stability with the logistic-Bernoulli units but not with ReLU.
%With ReLU activations this is not the case. 
%Parameter var=$0.1$ is the input variance.
\label{fig:LeNet}}
\end{figure}
%
%
\paragraph{Learning Speed and Normalization}
The goal of this experiment is to verify that our normalization has a similar positive impact on learning speed as batch normalization for stdNN in deeper networks where vanishing gradients pose a problem.
%We verify that our computed estimates can be used for normalization instead of real statistics and help with .
For this we consider a fully connected network with 6 layers of logistic transform units, 20 in each. %, which is difficult enough to test normalization. %Not a good architecture, arguably, but difficult enough to test normalization.
Using logistic {\em transform} units together with a very small input variance in varNN ensures that the network is deterministic 
%a We used a very small input variance for varNN to ensure that 
and that the forward passes of stdNN and varNN are nearly identical. The models and the corresponding likelihoods are then directly comparable. % as a consequence. %The networks are learned on MNIST data and the learning curves are shown in Fig.~\ref{fig:learnspeed}. 
Learning curves on MNIST data are shown in~\cref{fig:learnspeed}. It is clearly seen that without normalization both stdNN and varNN perform the same, as expected. With normalization varNN performs even better than stdNN with batch normalization. 
However, the validation accuracy curves indicate that a higher convergence rate is not necessarily an advantage if the overfitting is not controlled. We also tested the variant (V-Init), in which the normalization is performed for one iteration only and is frozen from then on, related to the initialization method~\cite{Mishkin-16-Init}. %, which efficiently provides a good initialization point, similarly to layer-sequential initialization~\cite{Mishkin-16-Init} but with our analytic estimates of statistics.
%%=============================================================================
\paragraph{Different Activations and Deeper CNNs}
%With a single layer network we have shown 
%\cite{Lecun-01}
We address the question whether the stability observed in a single layer network holds also in more general networks.
We consider a LeNet type network~\cite{Lecun-01} (4 layers, convolutions with strides) on MNIST with either ReLU or logistic-Bernoulli activations. In both cases varNN is more stable against Gaussian noise when compared with stdNN,~\cref{fig:LeNet}. The logistic-Bernoulli version of varNN is also more stable against adversarial attacks. This is not the case for the networks with ReLU units.
The learning procedure included model selection based on validation loss. The learning quickly overfits, with ReLU variant overfitting more (see loss plots in supplementary~\cref{fig:Lenet-losses-B,fig:Lenet-losses-R}). We believe this overfitting problem prevents good generalization in terms of stability. The optimization algorithm may drift in various directions depending, \eg, on model parametrization, \etc, of which we have no control.
\par
%We attempted scaling of our method to a somewhat larger network and dataset. Towards this end we tested 
Towards further scaling of the method we trained a conv network with 9 layers and logistic-Bernoulli activations on CIFAR dataset. The results in~\cref{fig:CIFAR} indicate that while varNN is more stable than stdNN, on the absolute scale it is still very sensitive to noise and perturbations. This challenge is left for future research.
%
%
%After proving superiority of varNN w.r.t.~to perturbation stability for a single layer and proving the positive impact of normalization on learning speed, we consider a CNN with four convolutional layers (similar to LeNet) and learn it on MNIST data. The goal is to analyze whether the stability of varNN w.r.t.~perturbations extends to deeper networks. Similar to the first experiment, we learned two variants of stdNN with and without batch normalization and two corresponding variants of varNN. We compared the results both for sigmoid logistic units and for ReLU units. In both cases varNN is more stable against unspecific noise with normal distribution when compared with stdNN. The sigmoid logistic version of VarNN is also more stable against adversarial attacks compared to its stdNN counterpart. This is not the case for the networks with ReLU units.
%
%Fig.~\ref{fig:LeNet} shows the learning convergence and the validation accuracy over learning epochs for the networks with sigmoid logistic units in two displays on the left and the stability comparison for Gaussian noise  and adversarial patterns in the two displays on right. It is clearly seen that the stdNN and varNN networks reach similar training/validations losses as well as similar validation accuracies. The differ however w.r.t. ~stability against perturbations. The corresponding comparison for the networks with ReLU units is given in the supplementary material.
%
%%
%
%
%
%


==> tex/normalization.tex <==
\paragraph{Normalization}
Batch normalization~\cite{IoffeS15} is a widely applied method that improves learning speed and performance of difficult networks. It is based on a whitening normalization, which requires computing the mean and variance statistics of all activations over the training set. In~\cite{IoffeS15} these statistics are approximated by those over a batch. {\em Layer normalization}~\cite{Ba-2016-Layer-Norm} uses statistics of different units within the same layer. Our model can instead compute an analytic estimate of such statistics in one pass. The idea is similar to self-normalizing networks~\cite{Klambauer-SELU}, where an analytical estimate of the mean and variance of an ELU unit is used to set the scaling and bias (once and for all) such that the output is normalized.

Assume that the training data have statistics $(\bar \mu^{0}, \bar\sigma^{0})$, which can be estimated prior to learning. varNN can be applied with these statistics on the input in order to estimate the statistics of activations $(\bar\mu^{k}, \bar\sigma^{k})$, depending on the current parameters. We do not claim these estimates to be accurate, but that they are suitable for normalization. We perform exactly the same reparametrization as proposed by~\cite{IoffeS15}: prior to non-linearity applying the transform:
\begin{align}\label{normalization}
\tilde X^k_i = (X^k_i - \bar\mu^k_i) / \bar\sigma^{k}_i \tilde s^k_i + \tilde b^k_i,
\end{align}
where $\tilde s^k_i$ and $\tilde b^k_i$ are new parameters, reintroducing a free scale and bias per channel so that the reparametrization does not change the degrees of freedom of the model. %Note that the transform affects both moments of $X^k$.
%

Similar to~\cite{IoffeS15}, during learning we need the values $(\bar \mu^{k}, \bar\sigma^{k})$ to be a part of the computation graph in order that~\eqref{normalization} is differentiated correctly. %This can be done by appending a "control sample" $(\bar \mu^{0}, \bar\sigma^{0})$ to any batch (possibly of size 1), which participates in all computations but the loss function. 
During testing, the normalizing values can be computed once and the network can be equivalently reparametrized back to the initial set of weights.
Differently from~\cite{IoffeS15} but similar to~\cite{Klambauer-SELU}, the statistics $(\bar\mu^{k}, \bar\sigma^{k})$ in the graph with normalization~\eqref{normalization} decouple over layers. Indeed, the normalization makes sure that $(X^k_i - \bar\mu^k_i) / \bar\sigma^{k}_i$ has zero mean and unit variance when the network input is $(\bar \mu^{0}, \bar\sigma^{0})$. Therefore, normalizing values $(\bar \mu^{k+1}, \bar \sigma^{k+1})$ of the next layer will depend only on $\tilde s^k$, $\tilde b^k$ and $W^{k+1}$ and not on the dataset statistics or the parameters of the preceding layers.
\par
%
%
We see the following advantages compared to~\cite{IoffeS15}: there is no dependence on batch size, the normalization is exactly the same during training and testing%(with BN the testing requires an up-to-date whole dataset statistics)
, we can easily convert between the initial model and the reparametrized one.


==> tex/unused.tex <==
\newpage
%\appendices
\appendix
\addtocontents{toc}{\protect\setcounter{tocdepth}{2}}
\pagestyle{plain}

%\title{\mytitle \\ Supplementary Material}
%\author{Authors}
%\maketitle

% Reset counters
\setcounter{figure}{0}
\setcounter{table}{0}
\counterwithin{figure}{section}
\counterwithin{table}{section}

% \title{\mytitle (CVPR'17 Appendix)}
\twocolumn[{%
 \centering
 \LARGE Some Unused Stuff \\[1.5em]
 \normalsize
}]

% TOC
% remove dots and page numbers
\let\Contentsline\contentsline
\renewcommand\contentsline[3]{\Contentsline{#1}{#2}{}}
\makeatletter
\renewcommand{\@dotsep}{10000}
\makeatother

\section{Brief Review of Probabilistic Models}\label{sec:prob-models}
There exist a certain gap between probabilistic models such as logistic belief networks~\cite{Neal:1992}, deep belief network~\cite{Hinton:2006-DBN}, \etc and feed-forward Deep Neural Networks (DNNs).
Probabilistic models specify full joint probability distribution over all states. 
%They can formalize a large variety of inference problems
They offer sound formulations for a large variety of inference problems: refining estimates of part of variables conditioned on any other part, generating samples, semi-supervised and unsupervised learning, \etc. Unfortunately, they have to deal with very difficult numerical estimation problems.
A line of such models is compared to DNN in~\cref{fig:models}, we also give a brief overview in~\cref{sec:prob-models}.

\begin{figure*}
\includegraphics[width=\linewidth]{fig/models-crop}
\caption{Illustration of different probabilistic models. 
\protect\begin{tabular}{c}
\includegraphics[height=2ex]{fig/node-image}
\protect\end{tabular}~%
Observed random variable (image).
\protect\begin{tabular}{c}
\includegraphics[height=2ex]{fig/node-latent}
\protect\end{tabular}~%
Posterior r. v. (segmentation).
\protect\begin{tabular}{c}
\includegraphics[height=2ex]{fig/node-hidden}
\protect\end{tabular}~%
Hidden r. v.
\protect\begin{tabular}{c}
\includegraphics[height=2ex]{fig/node-aux}
\protect\end{tabular}~%
Auxiliary variable (non-linearity).
\protect\begin{tabular}{c}
\includegraphics[height=2ex]{fig/line-undirected}
\protect\end{tabular}~%
Undirected graphical model (factorization of joint pdf).
\protect\begin{tabular}{c}
\includegraphics[height=2ex]{fig/line-directed}
\protect\end{tabular}~%
Directed graphical model (factorization of conditional probabilities), in DNN hidden layer forward propagation.
\label{fig:models}
}
%Deep Neural Network as a probabilistic model is closer to logistic regression with non-linear embedding.}
\end{figure*}
%
{\em Logistic regression} consists of a conditional probability model $p(Y\mid X)$ of a binary class $Y$ given observations $X$ and the maximum likelihood estimation. The form of the distribution $p(Y\mid X)$ is chosen such that the log likelihood ratio, which is the optimal Bayesian discriminant function, is linear in a certain feature space $\phi(X)$. The implied solution is that the distribution necessarily has the form $p(Y{=}1\mid X) = \S(w\T  \phi(X))$, where $\S$ is the logistic distribution function (popularly called sigmoid), $S(x) = 1/(1 + e^{-x})$.
\par
{\em Boltzmann machines} (BM) postulate joint probability distribution $p(X,Y)$ assuming both $X$ and $Y$ are binary (can be generalized by using appropriate embedding/lifting), as an exponential family $p(X,Y) \propto \exp(-E(X,Y))$. The energy $E(X,Y)$ of binary variables can be always represented in the form $E(X,Y) = X\T L X + a\T X + Y\T W X + b\T Y + Y\T R Y$. {\em Restricted Boltzmann machines} (RBM) do  not have the interactions inside the $X$ and $Y$ layers, \ie, restrict $L$ and $R$ to be zero.
%{\em Restricted Boltzmann machines} (RBM) postulate joint probability distribution $p(X,Y)$ assuming both $X$ and $Y$ are binary (can be generalized by using appropriate embedding/lifting), as an exponential family $p(X,Y) \propto \exp(-E(X,Y))$, where the energy $E(X,Y)$ of binary variables has the form $E(X,Y) = a\T X + X\T W Y + b\T Y$. 
It follows that given $X$, variables $Y_i$ and $Y_j$ in RBM are conditionally independent and the conditional distribution $p(Y_j{=}1 \mid X)$ expresses again as a logistic function $S(-W_j X - b_j)$. It holds symmetrically for $p(X_i \mid Y)$. RBMs can be trained using conditional likelihood and has proven to be quite rich generative models, although they are single layer.
\par
{\em Deep Belief Networks} (DBN)~\cite{Hinton:2006-DBN} have an RBM in the final two layers and more shallow layers are build conditionally on the deeper layers with conditional models $p(X^{k-1} \mid X^k)$ having the logistic form as shown in~\cref{fig:models}. Generating an image consists of sampling a state of RBM (more difficult) and generating from it more shallow layers like in Markov chain (easy). Solving recognition problems, sampling and evaluating probability are all difficult problems.
%combine a RBM on the two top hidden layers $X^l$, $X^{l-1}$ and a stack of conditional distributions $p(X^{k-1} \mid X^k)$, of the same form as the conditional distribution of an RBM, \ie conditionally independent models of $X^{k-1}_j$ given $X^{k}$ in the form $S({W^k_j}\T X^{k} + b^k_j)$.
Compared to the DCIM model~\eqref{DCIM}, DBNs assume conditional independence in the opposite direction. They model $p(X^l, X^{l-1})$ by a RBM and then stack conditionally independent distributions $p(X^{k-1} | X^{k})$ down to the image $X^0$, which forms a joint pdf of all states $p(X^l, X^{l-1},\dots, X^0)$, \eg, a full generative model. The model~\eqref{DCIM} is a directed graphical model, conditional on the input $X^0$.
\par
{\em Belief networks} (same as {\em Bayesian networks} or directed graphical models). Somewhat confusing, they have been considered prior to DBNs specifically with logistic activations (\eg,~\cite{Neal:1992}) and with a general number of layers, \ie, were already generally deep. DCIM model~\cite{Flach-17} with logistic layers is equivalent to logistic belief network~\cite{Neal:1992}.
\par
{\em Deep Boltzmann Machines}~\cite{salakhutdinov09a} are undirected graphical models that stack RBMs. %, \ie, that do not make a conditional independence assumption.
Generating a state of DBM does not decompose over cascades and poses a difficult problem. Is was shown nevertheless in~\cite{salakhutdinov09a}and subsequnt works that models with 2-3 hidden layers are powerful generative models which can be trained in a supervised fashion.
\par

%In {\em Deep Neural Networks} with sigmoid activations, the outputs of sigmoid activations of inner layers are often freely interpreted as posterior probabilities of occurrence of low-, mid- and high level visual features. However such interpretations are purely speculative because they are based solely on the fact that that outputs in all levels are numbers in the domain $[0, 1]$ and hence can represent some probabilities. Since there is no underlying probabilistic model, this interpretation can be neither proved nor disproved. The way how probabilistic outputs of one layer are transformed to that of the next layer is not derived from any joint model and they should be interpreted just as non-linearities. Only for the final layer the asymptotic consistency of the maximum likelihood guarantees estimation of the posterior probability of the data provided that the model capacity and amount of training data are large enough. Thus DNN can be viewed as logistic regression with non-linearly mapped inputs, where the mapping is also learned.
%%Our DCIM model allows full probabilistic interpretation. Main building blocks of DNNs: the sigmoid and softmax activations of linear mappings of inputs are _derived_ from DCIM model just for free under a simple approximate Bayesian inference. This allows to quantify probabilistic interpretations, look for better approximations, formulate generative and semi-supervised learning problems (as the demonstrated in our second contribution), etc. Hopefully, this clarifies the question what we mean by "closing the gap".
%%
%%
%%In {\em Deep Neural Networks} with sigmoid activations, hidden units are often interpreted as hidden random variables recognizing low-, mid- and high level visual features, increasingly abstract as the depth increases. Respectively, the outputs (activations) of inner layers are interpreted as posterior probabilities of visual feature occurrences. However these interpretations are purely speculative because they are based solely on the fact that that outputs in all levels are numbers in the domain $[0, 1]$ and hence can represent some probabilities. Since there is no underlying probabilistic model, this interpretation can be neither proved or disproved. The way how probabilistic outputs of one layer are transformed to that of the next layer is not derived from any joint model and they are understood just as non-linearities. Only for the final layer the consistency of the maximum likelihood guarantees estimation of the posterior probability of the data provided that the model capacity and amount of training data are large enough.
%%
%%A correct model 
%%be backed up by a probabilistic model explaining how these conditional probabilities are connected to each other 
%%however this is not supported by an underlying probabilistic model. 
%%In addition, performance of NNs with sigmoid activations is significantly hindered by problems with diminishing gradients during learning.
%%The output(s) is interpreted as posterior probability of a class label, but there is no theoretical clarity with respect to how probabilistic interpretation of hidden units is relevant for the output units.  
%%Deep neural networks with sigmoid activations are considered as very appealing models, however their performance is hindered by problems with diminishing gradients during learning. 
%\par
%%A recent work~\cite{Flach-17} shows that DNNs can be interpreted as deep conditional independent models (DCIM) with conditional distributions same as in RBMs stacked similarly to Deep Belief Networks but in the direction from image to hidden layers and that the standard forward computation procedure in NNs corresponds to a very simple approximate posterior inference in DCIM.
%\citet{Flach-17} recently proposed a deep conditional independent model, in which all units are discrete random variables, connected by logistic conditional distributions in the direction from the image to the hidden states. They showed that DNN forward computation can be viewed as a simple approximate Bayesian inference in this model. In this work we refine the accuracy of this approximation, yielding a new type of neural networks with improved properties.
%

\subsection{Deep Conditional Independent Model}
\citet{Flach-17} recently proposed a deep conditional independent model (DCIM), which specifies probability distribution of all hidden units using a chain of conditional logistic models.
%, in which all units are discrete random variables, connected by logistic conditional distributions in the direction from the image to the hidden states. 
They showed that a simple approximate Bayesian inference in this model replicates the known forward propagation in DNNs with sigmoid, $\tanh$ and softmax activations. In this work we extend the DCIM model by more general conditional models and propose more accurate approximations, yielding a new type of neural networks with improved properties.
%
%Following~\cite{Flach-17}, we consider the deep conditionally independent model. 
\par
The following extension of DCIM is considered. 
There are $l$ layers of hidden random variables $X^k$, $k=1,\dots l$ and $X^0$ is the input layer. For simplicity, we assume each layer has $n$ units.
\begin{definition}
%The layers are coupled together by pdf conditioned on $X^0$:
Deep conditional independent model is the pdf $p(X^{1,\dots l} \mid X^0)$ of all layers given the input layer $X^0$ such that it factors as 
\begin{align}\label{DCIM-old}
p(X^{1,\dots l} \mid X^0) = \textstyle \prod_{k=1}^{l} p(X^k \mid X^{k-1})
\end{align}
and probabilities $p(X^k \mid X^{k-1})$ satisfy conditional independence property for all $k$: variables $X^k_i$ and $X^k_j$ are conditionally independent given $X^{k-1}$ for all $i\neq j$.
%each variable $X^k_i$ in layer $k$ is conditionally independent from $X^k_j$ for $j\neq i$ given the states of all variables in the preceding layer $k-1$.
\end{definition}
DCIM is a Bayesian network, but without specifying a prior on $X^0$ and organized by layers. With logistic activations it matches the logistic belief net~\cite{Neal:1992}.
%
We allow both discrete and continuous random variables and several kinds of non-linearities and stochastic models. This ensures applicability and relevance of results in a wider context. %The following layers can be represented:
%Let us give several examples of layer activations that can be represented, denoting for clarity $p(Y\mid X)$ layer input as $X$ and the output as $Y$:
Let us give several examples of conditional models $p(Y\mid X)$, where we denoted two consecutive layers as $X,Y$:
%
\par\noindent$\bullet$\ {\em Logistic}: $Y_j$ is a binary discrete r.v. (takes values in $\{0,1\}$) and $p(Y_j \mid X)$ is the Bernoulli distribution with probability of $Y_j{=}1$ given by the logistic function $\S(w_j \T X)$. The input vector $X$ may be either binary or continuous.
%
\par\noindent$\bullet$\ {\em Non-linear transforms}:
$Y_j$ is a continuous variable, $p(Y_j \mid X)$ takes the form of a functional mapping, for example $p(Y_j{=}y \mid X)  = \delta\{ y {=} {\rm ReLU}(w_j\T X) \}$, which non-linearly transforms the input, \ie is deterministic given the input.
%
\par\noindent$\bullet$\ {\em Multinomial logistic (stochastic softmax)}: $Y_j$ is a discrete variable with two or more states and $p(Y_j{=}y \mid X) = \exp( w_y \T X) / \sum_k \exp( w_k \T X)$, \ie, the conditional distribution is given by the softmax function.
%
\par\noindent$\bullet$\ {\em Stochastic rectifier}: $Y_j = \max( 0, w_j \T X - Z)$, where $Z$ is an independent noise source.
Why this layer is a member of the family will be shown later on.
%, can be decomposed as non-linearity and noise.
%
\par\noindent
As can be seen, the extended model is sufficiently reach. %\citet{Flach-17} considered only discrete layers of the Bernoulli-logistic type.
%
%\par
%Layers that define a probability distribution will be called {\em stochastic}.
%
%When $X^k$ is a binary discrete variable, $p(X^k \mid X^{k-1})$ follow a logistic model 
%Thus, conditional probabilities $p(X^k \mid X^{k-1})$ can either follow a logistic model with binary hidden units $X^k$ or represent a deterministic non-linearity functions with real-valued outputs, such as {\rm ReLU}, by letting $p(X^k \mid X^{k-1}) = \delta\{X^k = {\rm ReLU}(W X^{k-1}) \}$. 
%
%Deep belief networks have a similar directed structure in all but the top layers, however the conditional independence is assumed in the opposite direction. They model the joint distribution $p(X^l, X^{l-1})$ by a restricted Boltzmann machine (undirected model) and then 
%

\subsection{(Old) Contribution}
In the extended DCIM model we consider the problem of approximate Bayesian inference of posterior probabilities $p(X^k_j \mid X^0)$ of hidden unit $X^k_j$ given the input image $X^0$. The approximate posterior $p(X^k_j \mid X^0)$, in the Bayesian view, represents a more complete information about the inferred state $X^k_j$ than a point estimate in~\cite{Flach-17}, equivalent to standard NN procedures. Towards this end we estimate the mean and variance of the posterior. For transform layers, this is equivalent to just propagating uncertainty in NNs as considered in~\cite{AstudilloN11} for logistic non-linearity. 
We derive new approximations for logistic and softmax conditional models, exploiting the fact that these probabilistic layers can be represented as composition of added noise and a non-linearity.
%For logistic model, we derive an approximation better than~\cite{Flach-17} and as accurate but simpler than~\cite{AstudilloN11}. 
We further derive / pull from the literature appropriate approximations to a number of non-linear transforms, yielding a family rich enough to allow uncertainty propagation in the state-of-the art NN models.
\par
The new model enjoys a number of useful properties. It is more accurate in estimating logical expressions under uncertain inputs and, more generally, less susceptible to making overconfident wrong predictions under perturbations~\cite{Moosavi-Dezfooli_2017_CVPR,Fawzi-16-robustness,Szegedy-14-intriguing,nguyen2015deep,Rodner16_FRN}.
It has self-normalization properties, related but principally different to batch normalization~\cite{IoffeS15} and self-normalizing networks~\cite{Klambauer-SELU} and can track the co-variate shift numerically without collecting statistics over data. Even with discontinuous non-linearities it has continuous gradients provided that there is some uncertainty. It automatically smooths-out non-linearities of more uncertain units, allowing better gradient propagation.
%There are further interesting possibilities, such as training with uncertain inputs, \etc.
%
\paragraph{(Old) Limitations} The framework is applicable for models that are suitable for recognition problems, when there is a single true value or class to estimate. A single-mode factorized distribution around the estimate simply provides a mean to more accurately assess the uncertainty of such estimates. %This has to be compared to a single point estimation provided by classical NNs. 
Models that generate e.g. images as their outputs usually have a multi-modal posterior distribution. In this case our simple approximation is not applicable as it cannot capture multiple modes.

%\paragraph{Limitations} Our approximation still assumes that parent variables $X_{pa(i)}$ for each $i$ are independent conditioned on the network input. In fact, we will introduce the approximation by considering a fully factorized posterior distribution. We believe such approximation is meaningful in settings where a point estimate is applicable applied. For example, when there is single correct answer in the estimation or classification problem.
%The framework is applicable for models that are suitable for recognition problems, when there is a single true value or class to estimate. A single-mode factorized distribution around the estimate simply provides a mean to more accurately assess the uncertainty of such estimates. %This has to be compared to a single point estimation provided by classical NNs. 
%Models that generate e.g. images as their outputs usually have a multi-modal posterior distribution. In this case our simple approximation is not applicable as it cannot capture multiple modes.

\subsection{(old) Approximation for Logistic Units}\label{binary-case}

In DNNs with logistic (sigmoid) activations, outputs of inner layers are often freely interpreted as posterior probabilities of occurrence of low-, mid- and high level visual features. However such interpretations are speculative because they are based solely on the fact that that outputs in all levels are logistic functions, \ie, numbers in the range $[0,1]$. There is no joint underling probabilistic model connecting them together. %Therefore, the probabilistic interpretation cannot be verified and no useful consequences from this interpretation can be derived.
Respectively, very little if anything at all can be verified or derived from this interpretation.
%
%Since there is no underlying probabilistic model, this interpretation can be neither proved nor disproved. 
%Nor it implies any useful recommendations, because these ``probabilities'' are not related to each other. 
The layered application of the logistic model to such ``probabilities'', not being derived from a joint latent variable model, can be interpreted as just a non-linear transform.
% %The way how outputs of one layer are transformed to that of the next layer, as not derived from any joint probability model and  should be interpreted just as a non-linear transform. 
Only for the final layer, asymptotic properties of the maximum likelihood estimator guarantees a consistent estimation of the posterior probability of the data provided that the model capacity and amount of training data are large enough. 
Therefore, as a probabilistic model, DNN can be viewed rather as a logistic model with non-linearly mapped inputs, where the mapping is also learned. Respectively, there are no recommendations from this model of how to pose such tasks as refining prediction based on some additional information, \eg in a multi-task network.
\par
%
A case of special interest is logical reasoning with uncertain inputs, such as "if we see car wheel with probability 50\% and car roof with probability 30\% what is the probability that the two parts are present simultaneously?". We will give an example showing that standard NN model with logistic unit has difficulties estimating it accurately, while a simple logistic probabilistic model does not.
%

\subsection{Binary}

\subsection{Non-vanishing gradients in Var-NN}
Consider the logistic unit. Let $\mu_i = \E [X_i ]$, $\sigma^2_i = \Var [X_i]$ denote the input and let the output of the linear transform be $\tilde \mu = w\T \mu + b$ and $\tilde \sigma^2 = \sum_i w_i^2 \sigma_i^2$.
%\par
%Under the standard approximation~\eqref{AP1}, let $\mu'$ denote its output, % = \S(w\T \mu+b)$ the output. %, $w\T \mu$
Let $\mu'$ denote the output of the standard approximation~\eqref{AP1}. The gradient in $w$ is given by
% with input $(w\T \mu + b, \sigma^2)$.
\begin{align}\label{AP1-g}
g_{\mu'} \frac{\d \S(\mu')}{d w}  = g_{\mu'} \S'(\mu') \mu, % = \frac{e^{-\mu}}{(1+e^{-\mu})^2}g_{\mu'},
\end{align}
where $g_{\mu'} = \d R / \d \mu'$ is the total derivative of the objective $R$ in the layer output $\mu'$. % (input of the backward pass).
%The asymptote is $e^{-|x|}$ for $|x|\rightarrow -\infty$ and the gradient quickly vanishes when $\mu$ is far away from zero. 
The gradient vanishes when $\mu'$ is large because the logistic density $\S'(\mu')$ vanishes at rate $e^{-|\mu'|}$. Good initialization and batch normalization help to prevent this by keeping $\mu' = w\T \mu +b$ low on average over the data.
\par
Now, let $\mu'$ and $\sigma'^2 = \mu'(1-\mu')$ be the output under the approximation~\eqref{AP2a}. The gradient in $w$ is given by
%
\begin{align}
%g_{\mu'} \frac{\d \Phi(\mu / \sqrt{\sigma^2+\pi^2/3})}{d \mu} + g_{\sigma^2'} \frac{\d \Phi(\mu / \sqrt{\sigma^2+\pi^2/3})}{d \mu}
g_{\mu'} \frac{\d \mu' }{\d w} + g_{\sigma'^2}\frac{\d \sigma'^2 }{\d w}  = 
\big(g_{\mu'} + g_{\sigma'^2} (2\mu'-1) \big) \frac{\d \mu' }{\d w},
\end{align}
and
\begin{align}
\frac{\d \mu' }{\d w} = \phi\Big(\frac{\tilde \mu}{\scriptstyle \sqrt{\tilde \sigma^2+\sigma_\S^2}}\Big) \frac{\d }{\d w} \frac{\tilde \mu}{\scriptstyle \sqrt{\tilde \sigma^2+\sigma_\S^2}}.
\end{align}
We see again that the gradient has exponential multiplier $\phi\Big( \tilde \mu / \scriptstyle \sqrt{\tilde \sigma^2+\sigma_\S^2}\Big)$.
If the uncertainties of the input $X$ are low, $\tilde \sigma^2$ is small and the denominator approaches constant. In this case the same effect as with~\eqref{AP1} is observed: gradient quickly vanishes when $\tilde \mu = w\T \mu + b$ is large. However, if the uncertainties are sufficiently high, they lead to automatic smoothing. More specifically,
\begin{proposition} Assume $X_i$ are Bernoulli and $\sigma^2_i \geq \alpha^2$ (satisfied for example, when $\mu_i \in [2\alpha^2, 1-2\alpha^2]$).
Then
\begin{align}\label{vanish-bound}
| \tilde \mu / \sqrt{\tilde \sigma^2+\sigma_s^2}| \leq \sqrt{\frac{\|w\|^2+b^2}{\|w\|^2\alpha^2+\sigma_S^2}}.
\end{align}
\end{proposition}
\begin{proof}
The square of nominator can be upper bounded as $|\tilde \mu|^2 = |w\T \mu + b|^2 \leq |w\T \mu|^2 + b^2 \leq \sum_{i}(w_i \mu_i)^2 + b^2 \leq ||w||^2 + |b|$.
The square of denominator can be lower bounded using $\tilde \sigma^2 = \sum_{i}w_i^2 \sigma_i \geq \sum_{i}w_i^2 \alpha^2  = ||w||^2 \alpha^2$. The claimed inequality follows.
\end{proof}
This shows that when ratio $\|w\| \gg |b|, 1$ there there is a constant portion of gradient that still does not vanish. 

This shows that when the bias $b$ is not too high compared to $||w||$, the uncertainty ensures that the exponential multiplier does not vanish and some constant portion of the gradient is potentially propagated, depending on other (non-exponential) factors in $w,b$. Note that inequality~\eqref{vanish-bound} is not tight, \eg for $\alpha=1/2$ there holds $|| \tilde \mu / {\tilde \sigma}|| \leq 1 + |b|/ ||w||$.
%

\subsection{Variational derivation of AP1}\label{AP1-variational}
This is an alternative derivation of~\cref{AP1}, which may be relevant to several works using variational approaches.
%
\par
Consider the following approximation for the marginal $p(Y)$, for the conditional model $p(Y \mid X) = \frac{1}{Z(X)}\exp(U(X,Y))$, where $U(X,Y) = \sum_{i,j}u_{i}(X_i,Y)$.
Let us write $p(Y \mid X)$ as $\exp(U(X,Y) - \log Z(X) )$. We then have the following inequality:
\begin{align}\label{approx-LB-exp}
p(Y) = &\sum_{x}p_X(x) \exp\Big\{ U(x,Y) - \log Z(x) \Big\} \\
\notag
\geq & \exp \Big\{\sum_{x}p_X(x) \big(U(x,Y) - \log Z(x) \big)\Big\},
\end{align}
which follows from Jensen's inequality for a convex function $\exp$. The approximation is obtained then by re-normalizing lower bounds~\eqref{approx-LB-exp} to define a proper distribution of $Y$:
\begin{align}
p_Y(y) \approx \frac{1}{Z} \exp\Big\{\sum_{x}p_X(x) U(x,y)\Big\},
\end{align}
where $Z = \sum_{y}\exp\{ \sum_{x}p_X(x) U(x,y) \}$. Notice that the complicating term $\sum_{x}p_X (x)\log Z(x)$, which does not depend on $y$ has canceled in this normalization. Finally, $\sum_{x}p_X(x) U(x,y)$ expresses as 
\begin{align}
\sum_{x}p_X(x) \sum_{i}u_{i}(x_i,y) = \sum_{i} \sum_{x_i}p(x_i) u_{i}(x_i,y).
\end{align}
%

\section{More}
\begin{lemma}\label{LAPNNbad}
The approximation~\eqref{AP1} denoted as $\hat p$ can be arbitrary far from the true marginal denoted as $p$ in the sense that for any $\alpha$ in $[0,1)$ there is a setting of parameters such that $|\hat p -p| > \alpha$.
\end{lemma}
\begin{proof}
\revisit todo
\end{proof}

\section{Discussion and Future Work}
%
NNs with binary random units are also very interesting in the connection with NNs with hard activations. Our inference procedures can be applied at training time and at test time units can be sampled taking values $\{0,1\}$ at random according to their conditional distributions. With binary outputs the application of linear filters is significantly simplified, while at the training time the model is differentiable. This is in contrast with methods where sampling is used during training and at test time deterministic thresholding or randomized thresholding not corresponding to the model is applied~\cite{CourbariauxB16}.
% can be applied at test time for efficiency purposes. 
%This replaces the need to calculate expectations with sampling from the conditional distribution and  In this scenario our method can be viewed as an estimator of the gradient in network with hard activations. 
Repeated sampling from the forward model should match in the expectation to our computed statistics, we believe this will yield a more accurate training method than the popular straight-through estimator~\cite{Bengio2013EstimatingOP}.
%\par
\par
Generative models of a more general form than composition of non-linearity with additive noise can be constructed as $Y = f(X,Z)$, where $Z$ is a noise source and $f$ is a fixed function. An example of such model is $p(Y \mid X)$ $\sim$ Normal with mean and variance given by the two-component input $X$, the model occurring in VAE~\cite{KingmaW13}.

